Enhancing Hallucination Detection through Perturbation-Based Synthetic Data Generation in System Responses

Detecting hallucinations in large language model (LLM) outputs is pivotal, yet traditional fine-tuning for this classification task is impeded by the expensive and quickly outdated annotation process, especially across numerous vertical domains and in the face of rapid LLM advancements. In this study, we introduce an approach that automatically generates both faithful and hallucinated outputs by rewriting system responses. Experimental findings demonstrate that a T5-base model, fine-tuned on our generated dataset, surpasses state-of-the-art zero-shot detectors and existing synthetic generation methods in both accuracy and latency, indicating efficacy of our approach.

==> sections/related_work.tex <==
\subsection{Close-source hallucination detection datasets}

\subsection{Close source hallucination detection benchmarks}



\subsection{Perturbation-based Hallucination Generation}

People have investigated several strategies to create hallucinations from a faithful text. 
For examples, FEVER~\cite{thorne2018fever} specified six types of mutation: paraphrasing, negation, substitution of an
entity/relation with a similar/dissimilar one, and
making the claim more general/specific and ask human to manually create unfaithful claims with these mutations.

Much prior work attempt to automatically create perturbations with or without human annotation.
In BEGIN~\cite{dziri-etal-2022-evaluating}, the author automatically generated hallucinations for training. They use two approaches to generate hallucinations. Firstly, they either swapped subject and object, or replaced named entities or verbs in the knowledge source, then ask a GPT2 based dialogue system to regenerate the response based on the new source, they found that these new responses tends to be hallucinated with respect to the original knowledge. Secondly, they tried to inject negations into the human response to create hallucination by leveraging synthetic parser and wordnet antonyms.
 It contains 

More recently,
HaluEval~\cite{} ask LLM to automatically replace entities with similar or dissimilar ones over OpenKGDial dataset with instructions and few-shot examples in their prompt.
~\cite{lucas-etal-2023-fighting} ask LLM to generate disinformation given faithful new articles and they define minor, major or critical perturbations in the prompt.
ICD~\cite{zhang2023alleviating} tries to mitigate LLM hallucinations by down-weighting the next token where a factually weak LLM will predict.  To construct a factually weak LLM, they finetuned LLM over some generated non-factual samples. They employ chatgpt to automatically convert factual samples from existing datasets into non-factual ones using instructions and few-shot prompts. The instructions and few shot examples are mainly about entity perturbation.

%The hallucination term has seen increased interest both publicly \footnote{\url{https://www.cam.ac.uk/research/news/cambridge-dictionary-names-hallucinate-word-of-the-year-2023}} and commercially \cite{rebedea2023nemo}.

